Tucker Tensor analysis of Matern functions in spatial statistics

In this work, we describe advanced numerical tools for working with multivariate functions and for the analysis of large data sets. These tools will drastically reduce the required computing time and the storage cost, and, therefore, will allow us to consider much larger data sets or finer meshes. Covariance matrices are crucial in spatio-temporal statistical tasks, but are often very expensive to compute and store, especially in 3D. Therefore, we approximate covariance functions by cheap surrogates in a low-rank tensor format. We apply the Tucker and canonical tensor decompositions to a family of Matern- and Slater-type functions with varying parameters and demonstrate numerically that their approximations exhibit exponentially fast convergence. We prove the exponential convergence of the Tucker and canonical approximations in tensor rank parameters. Several statistical operations are performed in this low-rank tensor format, including evaluating the conditional covariance matrix, spatially averaged estimation variance, computing a quadratic form, determinant, trace, loglikelihood, inverse, and Cholesky decomposition of a large covariance matrix. Low-rank tensor approximations reduce the computing and storage costs essentially. For example, the storage cost is reduced from an exponential $\mathcal{O}(n^d)$ to a linear scaling $\mathcal{O}(drn)$, where $d$ is the spatial dimension, $n$ is the number of mesh points in one direction, and $r$ is the tensor rank. Prerequisites for applicability of the proposed techniques are the assumptions that the data, locations, and measurements lie on a tensor (axes-parallel) grid and that the covariance function depends on a distance, $\Vert x-y \Vert$.

==> MATHS/PRE_MATH.TEX <==
%%%%% Begin  LaTeX  File PRE_MATH.tex             5. Feb. 96  %%%%%%%%%%%%%%%%%
%%%%%
%%%%% Definieren mathematischer Zusatzzeichen   und Symbole
%%%%%
%%%%%            based on HEADMATH.tex      Edgar Katzer, Hamburg, Sept. 1995.
%%%%%
%%%%%            and      AMMACROS.tex     (angewandte Mathematik Hamburg) 10. 11. 89
%%%%%                     PRE_VOSS.tex      H. VOSS, Sven Loges (9/89, 10/89) Mathematik TU-Harburg
%%%%%
%%%%% Author:    Edgar Katzer, Hamburg
%%%%% Version:   Version of 11. Dec, 1995,
%%%%%
%
%
%%%%%%%%%%%%%%%%%  Spezielle mathematische Zeichen       %%%%%%
%
%
%%  Mengensymbole
%
    \newcommand    {\BbbC}  {\mbox{\rm $\scriptscriptstyle    %%  complex C
                                   ^\mid$\hspace{-0.40em}C}}
    \newcommand    {\BbbN}  {\mbox{                           %%  integer N
                            \rm I\hspace{-0.22em}I\hspace{-0.32em}N}}
    \newcommand    {\BbbK}  {\mbox{                           %%  integer N
                            \rm I\hspace{-0.22em}I\hspace{-0.32em}K}}
    \newcommand    {\BbbQ}  {\mbox{\rm $\scriptscriptstyle    %%  rational Q
                                   ^\mid$\hspace{-0.40em}Q}}
    \newcommand    {\BbbR}  {\mbox{\rm I\hspace{-0.22em}R}}   %%  real    IR
    \newcommand    {\BbbE}  {\mbox{\rm I\hspace{-0.22em}E}}   %%  euclidian IE
    \newcommand    {\BbbZ}  {\mbox{\sf Z\hspace{-0.44em}Z}}   %%  integer Z

    \newcommand    {\icom}  {\BbbC}                           %%  complex C
    \newcommand    {\inat}  {\BbbN}                           %%  integer N
    \newcommand    {\irat}  {\BbbQ}                           %%  rational Q
    \newcommand    {\iree}  {\BbbR}                           %%  real    IR
    \newcommand    {\znat}  {\BbbZ}                           %%  integer Z

    \newcommand    {\nin}   {\in \hspace{-0.80em} /}       %%  not in
%
%   from  AMMACROS.tex   10.11.89
%
 %  \def            \R      {\mbox{\makebox[.2em][l]{I}R}}
 %  \def            \B      {\mbox{\makebox[.2em][l]{I}B}}
 %  \def            \N      {\mbox{\makebox[.2em][l]{I}N}}
 %  \def            \Z      {\mbox{\makebox[.22em][l]{\sf Z}{\sf Z}}}
               %\def\Z{\mbox{\makebox[.283em][l]{Z}Z}}
 %  \def            \C      {\makebox[.6em]{\makebox[-.18em]{C}\rule{.03em}{1.5ex}}}
               %\def\C{\makebox[.8em][l]{\makebox[.25em][l]{C}\rule{.03em}{1.5ex}}}
 %  \def            \Q      {\makebox[.6em]{\makebox[-.25em]{Q}\rule{.03em}{1.5ex}}}
               %\def\Q      {\makebox[.8em][l]{\makebox[.25em][l]{Q}\rule{.03em}{1.5ex}}}
    \def            \L      {\mbox{\makebox[.2em][l]{I}L}}
    \def            \P      {\mbox{\makebox[.2em][l]{I}P}}
%
%%  Spezielle Schriftarten  ( FETT,  \sf   etc
%
    \newcommand    {\ZZ}    { \mbox{\rm\bf{Z}} }
    \newcommand    {\HH}    { {^{\mbox{\scriptsize \sf H }}} }
    \newcommand    {\TT}    { {^{\mbox{\scriptsize \sf T }}} }
%
%
%%%%%%%%%%%%%%%%%  mathematische Begriffe                 %%%%%
%
    \newcommand    {\Bild}  { \mbox{\rm Bild$\,$} }
    \newcommand    {\Kern}  { \mbox{\rm Kernel$\,$} }
    \newcommand    {\Range} { \mbox{\rm Range$\,$} }
    \newcommand    {\Diag}  { \mbox{\rm diag$\,$} }
    \newcommand    {\cond}  { \mbox{\rm cond} }
    \newcommand    {\Span}  { \mbox{\rm Span$\,$} }

    \newcommand    {\Ccone} { \mbox{\rm CCone$\,$} }
    \newcommand    {\cone}  { \mbox{\rm cone$\,$} }
    \newcommand    {\grad}  { \mbox{\rm grad$\,$} }
    \newcommand    {\even}  { \mbox{\rm even$\,$} }
    \newcommand    {\odd}   { \mbox{\rm odd$\,$} }
    \newcommand    {\sonst} { \mbox{\rm sonst$\,$} }
%
%
%%%%%%%%%%%%%%%%%  Spezielle aufwendigere neue Zeichen   %%%%%%
%
%
    \newcommand    {\C}     { \langle }
    \newcommand    {\Z}     { \rangle }

    \newcommand    {\Doe}   { \mbox{
                                \makebox[.2em][c]{$\circ$}---\makebox[.2em][c]
                                                 {$\bullet$}  }}
    \newcommand    {\doe}   { \mbox{
                                \makebox[.2em][c]{$\bullet$}---\makebox[.2em][c]
                                                 {$\circ$}   }}
%
    \newcommand    {\isotone}  {\unitlength1pt
                                    \begin{picture}(28,15)
                                        \put(8,1){  \vector(2,1){12}  }
                                    \end{picture}   }
%
    \newcommand    {\kreuz}[2] {\mbox{ \raisebox{-1.2ex}
                                  {$\stackrel {\stackrel{#2}
                                     { \displaystyle \times}  }
                                  {\scriptscriptstyle {#1}}$}}}
%
    \newcommand    { \lgo }[2] {\begin{array}[t]{c}
                                   \longrightarrow \\ {\raisebox{2ex}[-2ex]
                                      {$\scriptstyle #1 \to #2 $} }
                                \end{array} }
%
    \newcommand    {\tmid}[1]  {\raisebox{1.95ex}[-1.95ex] {#1} }
%
%%%%%
%%%%%
%%%%% End    LaTeX  File PRE_MATH.tex            11. Dec. 95  %%%%%%%%%%%%%%%%%
